Learning How to Optimize Black-Box Functions With Extreme Limits on the Number of Function Evaluations

We consider black-box optimization in which only an extremely limited number of function evaluations, on the order of around 100, are affordable and the function evaluations must be performed in even fewer batches of a limited number of parallel trials. This is a typical scenario when optimizing variable settings that are very costly to evaluate, for example in the context of simulation-based optimization or machine learning hyperparameterization. We propose an original method that uses established approaches to propose a set of points for each batch and then down-selects from these candidate points to the number of trials that can be run in parallel. The key novelty of our approach lies in the introduction of a hyperparameterized method for down-selecting the number of candidates to the allowed batch-size, which is optimized offline using automated algorithm configuration. We tune this method for black box optimization and then evaluate on classical black box optimization benchmarks. Our results show that it is possible to learn how to combine evaluation points suggested by highly diverse black box optimization methods conditioned on the progress of the optimization. Compared with the state of the art in black box minimization and various other methods specifically geared towards few-shot minimization, we achieve an average reduction of 50\% of normalized cost, which is a highly significant improvement in performance.

==> tables/results_batch_variation.tex <==
\begin{tabular}{|c|cc|cc|cc|cc|cc|cc|}
% \toprule
\hline
        Epochs & \multicolumn{2}{c|}{4} & \multicolumn{2}{c|}{8} & \multicolumn{2}{c|}{12} & \multicolumn{2}{c|}{16} & \multicolumn{2}{c|}{24} & \multicolumn{2}{c|}{32} \\ \hline
               &   Mean &    Std &   Mean &    Std &   Mean &    Std &   Mean &    Std &   Mean &    Std &   Mean &    Std \\ \hline
% \midrule
\hline
         HPFSO &  {\bf 0.308} &   0.269 &  {\bf 0.191} &   0.220 &  {\bf 0.144} &  0.194 & {\bf  0.114} &  {\bf 0.177} &  {\bf 0.073} &  {\bf 0.136} &  {\bf 0.048} &  0.121 \\ \hline
           CMA &  0.322 &  0.246 &  0.218 & {\bf 0.207} &  0.173 &  {\bf 0.191} &  0.147 &  0.177 &  0.098 &  0.137 &  0.064 &  {\bf 0.106 }\\ \hline
          HEBO &  0.366 &  0.312 &  0.238 &  0.266 &  0.178 &  0.231 &  0.139 &  0.202 &  0.101 &  0.175 &  0.073 &  0.155 \\ \hline
       ILSHADE &  0.427 &  {\bf 0.235} &  0.355 &  0.246 &  0.279 &  0.245 &  0.259 &  0.242 &  0.211 &  0.214 &  0.163 &  0.204 \\ \hline
       GBM-LCB &  0.462 &  0.343 &  0.333 &  0.289 &  0.285 &  0.271 &  0.248 &  0.252 &  0.214 &  0.234 &  0.191 &  0.221 \\ \hline
         SHADE &  0.410 &  0.302 &  0.357 &  0.272 &  0.327 &  0.271 &  0.285 &  0.249 &  0.270 &  0.247 &  0.216 &  0.223 \\ \hline
          SADE &  0.413 &  0.306 &  0.345 &  0.272 &  0.332 &  0.269 &  0.271 &  0.240 &  0.252 &  0.252 &  0.216 &  0.224 \\ \hline
           jSO &  0.415 &  0.300 &  0.357 &  0.278 &  0.311 &  0.266 &  0.297 &  0.264 &  0.254 &  0.236 &  0.221 &  0.230 \\ \hline
        LSHADE &  0.414 &  0.298 &  0.356 &  0.278 &  0.317 &  0.256 &  0.291 &  0.260 &  0.250 &  0.243 &  0.223 &  0.235 \\ \hline
 LSHADECNEP* &  0.398 &  0.301 &  0.343 &  0.263 &  0.325 &  0.267 &  0.309 &  0.256 &  0.262 &  0.241 &  0.237 &  0.236 \\ \hline
            DE &  0.415 &  0.299 &  0.371 &  0.279 &  0.352 &  0.283 &  0.305 &  0.261 &  0.289 &  0.252 &  0.252 &  0.242 \\ \hline
           RER &  0.575 &  0.331 &  0.452 &  0.298 &  0.409 &  0.285 &  0.385 &  0.276 &  0.358 &  0.263 &  0.335 &  0.253 \\ \hline
         GGA++ &  0.603 &  0.323 &  0.486 &  0.309 &  0.425 &  0.291 &  0.395 &  0.281 &  0.370 &  0.281 &  0.337 &  0.265 \\ \hline
           REP &  0.601 &  0.316 &  0.485 &  0.295 &  0.436 &  0.283 &  0.399 &  0.280 &  0.360 &  0.274 &  0.338 &  0.269 \\ \hline
           TUR &  0.573 &  0.321 &  0.476 &  0.300 &  0.428 &  0.281 &  0.402 &  0.279 &  0.367 &  0.269 &  0.338 &  0.265 \\ \hline
           LHS &  0.580 &  0.328 &  0.486 &  0.297 &  0.441 &  0.283 &  0.405 &  0.275 &  0.365 &  0.263 &  0.342 &  0.258 \\ \hline
% \bottomrule
\end{tabular}


==> tables/results_batch_variation_norm.tex <==
\begin{tabular}{|c|cc|cc|cc|cc|cc|cc|}
% \toprule
\hline
        Epochs & \multicolumn{2}{c|}{4} & \multicolumn{2}{c|}{8} & \multicolumn{2}{c|}{12} & \multicolumn{2}{c|}{16} & \multicolumn{2}{c|}{24} & \multicolumn{2}{c|}{32} \\ \hline
               & Mean & Std & Mean & Std & Mean & Std & Mean &Std & Mean & Std & Mean & Std \\ \hline
% \midrule
\hline
         HPFSO &         {\bf 0.419} &         {\bf0.350} &          {\bf0.217} &         0.245 &          {\bf0.137} &         0.201 &          {\bf0.067} &         {\bf0.115} &         {\bf-0.068} &        1.123 &         -0.118 &         1.177 \\ \hline
           CMA &          0.477 &         0.408 &          0.265 &         {\bf0.219} &          0.177 &         {\bf0.189} &          0.142 &         0.207 &         -0.031 &         1.080 &         {\bf-0.159} &         1.486 \\ \hline
          HEBO &          0.825 &         2.434 &          0.345 &         0.570 &          0.200 &         0.252 &          0.135 &         0.199 &          0.073 &         {\bf 0.183} &          0.024 &        {\bf 0.167 }\\ \hline
       ILSHADE &          1.844 &        11.54 &          0.512 &         0.328 &          0.349 &         0.262 &          0.303 &         0.259 &          0.230 &         0.212 &          0.158 &         0.190 \\ \hline
       GBM-LCB &          0.670 &         0.481 &          0.450 &         0.351 &          0.365 &         0.320 &          0.341 &         0.317 &          0.251 &         0.255 &          0.212 &         0.236 \\ \hline
        LSHADE &         30.32 &       366.5 &          1.555 &        12.19 &          0.532 &         1.120 &          0.379 &         0.325 &          0.299 &         0.278 &          0.252 &         0.253 \\ \hline
          SADE &          0.811 &         1.385 &          0.672 &         2.061 &          0.478 &         0.478 &          0.343 &         0.274 &          0.303 &         0.288 &          0.242 &         0.222 \\ \hline
           jSO &         19.08 &       222.9&          9.327 &       108.6 &          9.683 &       115.9 &          0.384 &         0.321 &          0.322 &         0.323 &          0.249 &         0.253 \\ \hline
 LSAHDECNEP* &         39.80 &       487.3 &          1.530 &        12.197 &          0.521 &         0.893 &          0.410 &         0.313 &          0.325 &         0.280 &          0.426 &         1.838 \\ \hline
         SHADE &         23.30 &       281.6 &          0.635 &         1.560 &          0.460 &         0.414 &          0.365 &         0.302 &          0.334 &         0.288 &          0.243 &         0.240 \\ \hline
            DE &          2.227 &        16.92 &          5.708 &        61.93 &          1.173 &         8.582 &          0.410 &         0.326 &          0.370 &         0.300 &          0.307 &         0.292 \\ \hline
           REP &          1.246 &         1.709 &          0.818 &         0.807 &          0.691 &         0.748 &          0.543 &         0.311 &          0.483 &         0.311 &          0.444 &         0.303 \\ \hline
           RER &          8.014 &        85.32 &          0.710 &         0.543 &          0.600 &         0.389 &          0.549 &         0.336 &          0.494 &         0.322 &          0.454 &         0.300 \\ \hline
         GGA++ &          1.177 &         1.776 &          0.761 &         0.503 &          0.648 &         0.425 &          0.521 &         0.307 &          0.510 &         0.322 &          0.455 &         0.304 \\ \hline
           TUR &          1.119 &         1.506 &          0.753 &         0.545 &          0.633 &         0.354 &          0.534 &         0.304 &          0.518 &         0.331 &          0.453 &         0.304 \\ \hline
           LHS &          1.272 &         3.378 &          0.783 &         0.598 &          0.661 &         0.417 &          0.606 &         0.304 &          0.520 &         0.312 &          0.477 &         0.292 \\ \hline
% \bottomrule
\end{tabular}


==> tables/results_complete.tex <==
\begin{tabular}{lrrrrrrrrrrr}
\toprule
       instance &    HPFSO &        HEBO &         cma &     ilshade &      lshade &        sade &         jso &       shade &          de &  lshadecnepsin &       TURBO \\ \hline
\midrule
 f016\_i04\_d05 &    -512.05 &     -517.25 &     -503.08 &     -512.46 &     -507.51 &     -507.77 &     -508.82 &     -503.69 &     -502.64 &        -508.92 &     -507.93 \\ \hline
 f020\_i80\_d40 &    2633.91 &    27903.33 &     8488.18 &    53975.43 &    19972.30 &    10499.60 &    10938.29 &    21417.27 &    20989.54 &       16391.62 &   132934.19 \\ \hline
 f008\_i01\_d03 &     151.55 &      149.22 &      151.28 &      149.22 &      150.37 &      153.49 &      155.41 &      152.45 &      150.47 &         152.85 &      347.54 \\ \hline
 f017\_i74\_d10 &     -30.35 &      -26.93 &      -27.95 &      -16.87 &      -14.39 &      -18.01 &      -11.91 &      -16.44 &      -14.28 &         -12.99 &      -19.53 \\ \hline
 f018\_i05\_d05 &    -145.98 &     -128.30 &     -143.76 &     -131.92 &     -133.09 &     -134.08 &     -133.00 &     -128.62 &     -136.01 &        -129.21 &     -125.56 \\ \hline
 f018\_i04\_d40 &      71.63 &       85.01 &       84.76 &       87.34 &       79.08 &       77.77 &       79.32 &       76.12 &       77.69 &          79.10 &       99.40 \\ \hline
 f005\_i77\_d03 &     150.82 &      149.59 &      149.59 &      182.74 &      187.82 &      165.32 &      176.78 &      179.97 &      171.05 &         184.00 &      163.40 \\ \hline
 f002\_i72\_d20 &  158102.01 &    75119.29 &  1460471.44 &  2848986.65 &  4340262.06 &  2502305.25 &  3360758.11 &  4629952.13 &  3467224.72 &     4091189.00 &  2299094.08 \\ \hline
 f012\_i01\_d03 &    1151.89 &     -231.53 &     -520.09 &     -474.28 &   258762.10 &   204972.69 &      677.14 &     7456.62 &   130054.87 &       49880.32 &   565158.68 \\ \hline
 f019\_i04\_d10 &     -54.81 &      -58.23 &      -52.82 &      -55.07 &      -53.65 &      -54.24 &      -52.90 &      -53.41 &      -54.64 &         -54.04 &      -47.49 \\ \hline
 f020\_i01\_d03 &    -544.73 &     -544.48 &     -544.26 &     -545.94 &     -544.91 &     -544.31 &     -544.18 &     -544.17 &     -543.98 &        -543.49 &     -543.04 \\ \hline
 f015\_i80\_d20 &     404.78 &      522.16 &      428.70 &      574.95 &      570.94 &      668.72 &      619.42 &      602.46 &      657.21 &         614.86 &      979.57 \\ \hline
 f008\_i76\_d10 &    1194.40 &     1340.87 &     1220.85 &    16383.18 &    18871.35 &    15079.38 &    19326.61 &    12942.77 &    14096.67 &       18279.06 &    40566.46 \\ \hline
 f020\_i05\_d02 &      -5.74 &       -4.94 &       -5.02 &       -4.47 &       -5.59 &       -4.45 &       -6.29 &       -5.41 &       -6.12 &          -3.99 &       -5.35 \\ \hline
 f010\_i77\_d05 &    5457.04 &    24426.74 &     1720.34 &   333965.27 &   523981.48 &   242198.50 &   488401.24 &   572767.92 &   801974.11 &      382676.44 &    83927.63 \\ \hline
 f010\_i74\_d20 &  210079.29 &   394959.53 &   726094.08 &   359757.62 &   858922.07 &   871838.87 &   338991.14 &   897419.00 &   738316.30 &      604760.40 &  1092779.77 \\ \hline
 f009\_i05\_d40 &    9078.92 &      319.11 &     9257.76 &    98023.35 &     4608.53 &     3738.70 &     3739.00 &     3353.15 &     4880.49 &        3334.98 &   300558.93 \\ \hline
 f011\_i76\_d40 &     196.24 &      497.21 &     2142.53 &     1107.57 &      129.61 &      129.40 &       77.96 &      273.10 &      103.22 &          80.89 &      376.64 \\ \hline
 f007\_i05\_d02 &      64.80 &       64.83 &       64.80 &       64.79 &       64.83 &       65.42 &       64.80 &       64.80 &       65.42 &          65.42 &       64.90 \\ \hline
 f014\_i04\_d02 &      39.92 &       39.92 &       39.92 &       39.94 &       39.96 &       39.97 &       39.92 &       42.23 &       40.02 &          40.00 &       40.28 \\ \hline
 f010\_i05\_d05 &     241.08 &    29981.87 &    40305.49 &    15832.98 &    93936.25 &   467574.30 &   227532.48 &   260439.23 &   386205.77 &      109032.66 &    19758.39 \\ \hline
 f004\_i76\_d40 &     636.84 &      920.93 &      661.01 &     1272.56 &      706.47 &      735.26 &      744.58 &      638.00 &      751.91 &         695.69 &     2172.42 \\ \hline
 f018\_i76\_d05 &      50.15 &       51.54 &       54.66 &       48.86 &       52.84 &       54.28 &       56.78 &       57.11 &       61.37 &          53.84 &       55.93 \\ \hline
 f022\_i71\_d03 &     154.67 &      152.79 &      152.83 &      155.08 &      154.68 &      155.95 &      160.36 &      154.67 &      153.22 &         156.28 &      159.61 \\ \hline
 f014\_i74\_d02 &       7.73 &        7.64 &        7.64 &        7.66 &        8.96 &        7.80 &        7.71 &        7.68 &       10.21 &           8.22 &        7.87 \\ \hline
 f022\_i05\_d10 &      70.41 &       68.67 &       78.66 &       86.71 &      110.91 &      106.27 &       81.77 &       97.14 &      112.50 &         112.73 &      117.82 \\ \hline
 f010\_i73\_d10 &   23265.86 &   166301.97 &   206082.31 &   203127.03 &  2132592.75 &   426801.06 &   719298.28 &   475420.44 &  1230329.12 &     1060334.57 &   942759.21 \\ \hline
 f013\_i71\_d02 &      29.09 &       34.76 &       28.52 &       28.55 &       30.85 &       35.24 &       33.73 &       29.72 &       38.57 &          30.02 &       33.70 \\ \hline
 f020\_i73\_d10 &    -245.16 &     -244.80 &     -244.70 &     -244.40 &      237.85 &       51.52 &     -212.64 &     -245.11 &      642.41 &        -147.81 &     9341.85 \\ \hline
 f008\_i79\_d40 &   38013.69 &    75986.70 &    65611.22 &   143561.87 &    32113.48 &    53783.18 &    47697.33 &    48490.49 &    56842.17 &       52997.03 &   283658.51 \\ \hline
 f001\_i73\_d40 &    -514.39 &     -403.33 &     -479.46 &     -396.49 &     -448.34 &     -436.74 &     -440.20 &     -443.47 &     -430.08 &        -449.49 &     -281.91 \\ \hline
 f006\_i01\_d02 &      35.98 &       36.42 &       35.90 &       35.92 &       36.86 &       36.18 &       36.18 &       35.94 &       36.62 &          36.13 &       36.24 \\ \hline
 f010\_i79\_d02 &    -986.01 &     -990.32 &     -962.71 &     -980.27 &     -955.50 &     -703.83 &     -980.10 &     -966.05 &     -999.20 &        -927.94 &     -971.75 \\ \hline
 f010\_i76\_d20 &  372372.36 &  1083511.33 &  1075721.58 &   808660.40 &   843614.53 &  1551548.74 &  1113598.82 &  1341834.77 &   896259.80 &     1283210.91 &  2573125.36 \\ \hline
 f004\_i74\_d40 &     808.33 &     1197.57 &     1227.10 &     1625.29 &     1047.77 &      994.34 &     1005.78 &     1006.79 &     1011.19 &        1007.82 &     2858.47 \\ \hline
 f008\_i78\_d10 &    1047.95 &     1203.38 &     1176.76 &     2174.15 &     2930.18 &     2098.41 &     4670.98 &     2714.27 &     2127.84 &        2373.21 &    17146.04 \\ \hline
 f008\_i77\_d03 &    -676.89 &     -678.77 &     -678.92 &     -664.95 &     -594.74 &     -671.90 &     -667.70 &     -678.63 &     -655.21 &        -667.18 &     -465.54 \\ \hline
 f022\_i80\_d02 &    -305.86 &     -305.86 &     -305.86 &     -305.86 &     -305.82 &     -305.84 &     -305.86 &     -305.80 &     -305.51 &        -305.85 &     -306.02 \\ \hline
 f005\_i05\_d10 &     -16.97 &      -37.45 &      -31.57 &       95.14 &      115.39 &      111.05 &      131.52 &      116.11 &      120.28 &         107.50 &       35.68 \\ \hline
 f018\_i04\_d10 &      49.66 &       48.45 &       53.05 &       64.63 &       64.42 &       68.55 &       73.91 &       69.85 &       70.96 &          72.14 &       60.89 \\ \hline
 f006\_i80\_d10 &     -82.84 &      -10.23 &      450.67 &    73427.32 &   146292.66 &    69928.03 &   156853.36 &   101138.52 &   125442.69 &       96637.53 &    61142.58 \\ \hline
 f008\_i72\_d10 &     -54.56 &      -91.66 &      462.32 &      873.09 &     1976.05 &     2034.43 &     2084.13 &     1802.55 &     2093.74 &        2005.73 &     7906.45 \\ \hline
 f013\_i77\_d40 &    2122.71 &     3017.72 &     2076.70 &     2981.86 &     2913.84 &     3053.83 &     2913.33 &     2920.97 &     2938.01 &        2830.76 &     3257.58 \\ \hline
 f007\_i03\_d05 &       6.74 &        9.43 &        7.36 &       14.38 &       27.54 &       79.25 &      165.52 &       76.29 &       77.36 &          66.00 &       33.35 \\ \hline
 f010\_i01\_d03 &     115.04 &     1036.79 &      -17.71 &      -42.81 &      -25.21 &      632.49 &      109.96 &       53.35 &     2107.54 &         751.98 &    10067.99 \\ \hline
 f013\_i80\_d03 &     -41.36 &      -43.37 &       -8.53 &      -43.17 &      -32.96 &      -28.09 &      -40.04 &      -37.23 &      -39.19 &         -25.98 &       51.55 \\ \hline
 f003\_i01\_d03 &    -459.82 &     -460.03 &     -454.87 &     -450.41 &     -453.07 &     -445.50 &     -448.76 &     -451.64 &     -441.00 &        -421.52 &     -444.39 \\ \hline
 f011\_i78\_d40 &     347.11 &      670.96 &     2668.35 &      993.73 &      232.94 &      256.55 &      262.89 &      378.55 &      187.59 &         447.05 &      964.83 \\ \hline
 f009\_i71\_d02 &     935.02 &      934.95 &      935.57 &      934.82 &      934.84 &      935.10 &      934.86 &      934.93 &      934.86 &         934.88 &      936.31 \\ \hline
 f019\_i03\_d40 &     224.37 &      214.26 &      226.03 &      229.33 &      221.66 &      221.78 &      221.09 &      221.49 &      222.13 &         221.51 &      243.35 \\ \hline
 f023\_i72\_d20 &    1004.32 &     1005.25 &     1007.78 &     1004.62 &     1004.23 &     1004.46 &     1004.60 &     1003.55 &     1004.07 &        1003.81 &     1004.97 \\ \hline
 f022\_i01\_d05 &    -999.51 &     -994.43 &     -998.00 &     -999.53 &     -993.41 &     -992.58 &     -998.99 &     -998.02 &     -997.48 &        -991.49 &     -973.74 \\ \hline
 f005\_i80\_d03 &     -40.47 &      -40.96 &      -40.96 &      -10.44 &      -12.28 &      -24.59 &        1.14 &      -17.41 &        6.72 &          -2.79 &      -31.71 \\ \hline
 f013\_i79\_d40 &    1256.77 &     2104.25 &     1470.50 &     2140.12 &     1753.17 &     1703.81 &     1862.38 &     1924.78 &     1797.89 &        1760.51 &     3037.91 \\ \hline
 f010\_i02\_d10 &   96356.82 &    94541.40 &    16730.76 &  1227922.62 &  2067003.87 &  1638450.15 &  1465081.87 &   672849.39 &  1695007.36 &     2055240.61 &   356654.12 \\ \hline
 f023\_i03\_d10 &    -127.20 &     -127.91 &     -126.06 &     -126.94 &     -127.07 &     -125.26 &     -126.35 &     -126.73 &     -128.24 &        -126.69 &     -126.50 \\ \hline
 f022\_i03\_d10 &     -45.44 &        1.72 &      -22.10 &        9.51 &        6.96 &       -7.07 &       13.04 &       17.31 &        5.00 &          -6.17 &       11.25 \\ \hline
 f007\_i80\_d10 &    1012.62 &     1025.17 &     1047.83 &     1032.99 &     1043.52 &     1064.19 &     1047.96 &     1058.57 &     1054.07 &        1066.96 &     1048.93 \\ \hline
 f016\_i01\_d10 &      91.06 &       89.11 &       96.60 &       93.76 &       94.13 &       88.83 &       94.54 &       96.87 &       89.45 &          92.75 &      106.00 \\ \hline
 f005\_i74\_d02 &    -182.61 &     -183.02 &     -183.02 &     -155.70 &     -183.02 &     -170.21 &     -177.72 &     -179.75 &     -170.56 &        -156.38 &     -180.85 \\ \hline
 f007\_i05\_d40 &     443.28 &     1229.52 &      828.50 &     1419.79 &     1305.58 &     1391.20 &     1427.09 &     1382.11 &     1408.70 &        1310.10 &     2092.79 \\ \hline
 f006\_i04\_d02 &     133.06 &      133.99 &      132.25 &      132.30 &      134.48 &      132.86 &      135.78 &      133.10 &      132.63 &         133.27 &      133.21 \\ \hline
 f022\_i74\_d20 &      51.11 &       34.95 &       81.36 &       87.78 &       90.91 &       91.79 &       90.54 &       84.24 &       89.77 &          85.51 &       92.15 \\ \hline
 f011\_i79\_d40 &     724.00 &      631.46 &      541.81 &   301424.20 &  1609995.66 &   479838.19 &   595794.90 &   886537.09 &  1653688.44 &      154214.13 &    28333.59 \\ \hline
 f013\_i02\_d05 &      12.46 &       12.44 &       10.98 &      547.34 &      535.42 &      697.81 &      709.23 &      622.80 &      633.87 &         705.62 &      427.71 \\ \hline
 f010\_i05\_d10 &   35412.80 &    18710.22 &   110867.95 &   436335.91 &   545344.45 &   323347.67 &   517945.38 &   298364.48 &   804324.58 &      460768.92 &   370887.79 \\ \hline
 f015\_i78\_d03 &      63.89 &       53.65 &       59.94 &       65.92 &       67.09 &       91.00 &       80.29 &       75.80 &       74.41 &          84.04 &       81.49 \\ \hline
 f002\_i05\_d20 &  137401.76 &    81468.60 &   676400.15 &  3663500.68 &  6107495.38 &  5279088.28 &  5161081.55 &  7103280.52 &  5031651.04 &     4048577.38 &  1469275.83 \\ \hline
 f021\_i01\_d05 &      42.21 &       42.17 &       42.83 &       42.98 &       47.01 &       46.13 &       48.18 &       43.12 &       47.41 &          42.91 &       57.15 \\ \hline
 f015\_i79\_d02 &    -362.47 &     -362.13 &     -362.23 &     -359.96 &     -361.91 &     -355.29 &     -360.20 &     -358.38 &     -357.24 &        -354.27 &     -359.43 \\ \hline
 f013\_i74\_d40 &    1612.80 &     2401.93 &     1363.01 &     2508.12 &     2361.05 &     2348.70 &     2299.78 &     2416.81 &     2409.54 &        2403.66 &     3381.94 \\ \hline
 f013\_i75\_d10 &     176.58 &      193.09 &      336.53 &      598.21 &      630.02 &      615.35 &      792.01 &      638.30 &      678.40 &         649.73 &      755.66 \\ \hline
 f009\_i76\_d20 &    1254.15 &      118.66 &     1581.05 &     1009.26 &     1325.34 &     1413.57 &      980.61 &      978.07 &     1380.82 &        1421.92 &    78978.76 \\ \hline
 f014\_i02\_d03 &    -179.50 &     -179.53 &     -179.40 &     -179.52 &     -179.10 &     -178.85 &     -179.29 &     -178.13 &     -178.70 &        -178.69 &     -178.76 \\ \hline
 f005\_i04\_d10 &     956.55 &      941.67 &      941.67 &     1090.73 &     1104.76 &     1101.48 &     1107.43 &     1091.33 &     1099.03 &        1096.49 &     1052.34 \\ \hline
 f013\_i80\_d20 &     702.12 &     1431.79 &      833.15 &     1598.21 &     1659.33 &     1733.81 &     1732.76 &     1551.74 &     1702.47 &        1660.83 &     2006.95 \\ \hline
 f010\_i03\_d10 &   11948.15 &    53773.40 &    56529.06 &   137283.77 &   549549.05 &   200023.65 &   389626.10 &   152302.47 &   131245.59 &      604432.06 &   393889.54 \\ \hline
 f009\_i71\_d10 &     976.63 &      970.11 &     1219.03 &     1035.65 &     1000.98 &     1187.18 &     1171.25 &     1211.30 &     1179.18 &        1246.65 &    13984.32 \\ \hline
 f019\_i79\_d02 &      29.12 &       28.80 &       28.85 &       28.86 &       28.82 &       28.82 &       28.80 &       28.90 &       28.87 &          28.92 &       28.98 \\ \hline
\bottomrule
\end{tabular}


==> tables/results_complete_cont.tex <==
\begin{tabular}{lrrrrrrrrrrr}
\toprule
       instance &     HPFSO &        HEBO &         cma &      ilshade &       lshade &         sade &          jso &        shade &           de &  lshadecnepsin &        TURBO \\ \hline
\midrule
 f024\_i77\_d02 &       -9.03 &       -9.13 &       -9.82 &        -9.93 &        -5.09 &        -5.64 &        -8.75 &        -8.32 &       -12.47 &          -8.75 &        -5.45 \\ \hline
 f014\_i74\_d40 &       38.93 &       64.58 &       38.55 &        59.39 &        49.11 &        45.97 &        45.69 &        42.14 &        51.11 &          42.66 &        79.60 \\ \hline
 f015\_i02\_d40 &      923.10 &     1200.77 &     1002.62 &      1442.39 &      1256.57 &      1308.93 &      1371.70 &      1299.72 &      1128.55 &        1354.57 &      2208.74 \\ \hline
 f005\_i02\_d03 &      656.22 &      655.99 &      655.99 &       672.36 &       683.52 &       680.12 &       693.20 &       693.22 &       694.47 &         695.22 &       662.76 \\ \hline
 f019\_i77\_d20 &       -3.96 &      -10.10 &       -1.55 &        -3.84 &        -4.25 &        -4.05 &        -3.53 &        -3.73 &        -4.05 &          -3.98 &        14.12 \\ \hline
 f002\_i04\_d02 &      320.31 &      320.19 &      320.24 &       330.48 &       328.59 &       424.14 &       321.66 &      3150.92 &       321.32 &         425.90 &       413.13 \\ \hline
 f012\_i72\_d02 &      -39.33 &      -61.26 &      -85.21 &       -84.71 &       -84.66 &       118.38 &       -82.39 &        94.26 &       -83.59 &         299.93 &       -84.90 \\ \hline
 f007\_i74\_d05 &       93.49 &       97.31 &       94.18 &       101.98 &       112.98 &       119.01 &       115.58 &       120.94 &       100.96 &         110.01 &       105.34 \\ \hline
 f011\_i01\_d20 &      279.50 &      446.04 &      391.25 &       167.92 &       164.31 &       351.09 &       208.74 &       346.68 &       238.47 &         548.96 &       332.20 \\ \hline
 f014\_i74\_d10 &        9.86 &       10.85 &       12.80 &        17.62 &        23.62 &        24.74 &        25.16 &        20.96 &        25.35 &          21.43 &        27.90 \\ \hline
 f004\_i80\_d20 &      366.28 &      471.22 &      519.06 &       516.96 &       599.62 &       555.72 &       562.42 &       531.05 &       626.65 &         587.65 &      1092.20 \\ \hline
 f014\_i71\_d40 &       65.53 &      106.78 &       54.74 &        97.14 &        77.32 &        90.43 &        80.76 &        88.23 &        95.32 &          86.43 &        98.94 \\ \hline
 f019\_i77\_d40 &       -0.48 &      -10.10 &        0.89 &         4.41 &        -3.39 &        -2.77 &        -2.58 &        -3.38 &        -2.41 &          -3.49 &        16.03 \\ \hline
 f017\_i72\_d05 &      -34.58 &      -35.45 &      -35.74 &       -33.97 &       -33.21 &       -33.06 &       -32.03 &       -32.73 &       -31.95 &         -32.04 &       -30.98 \\ \hline
 f015\_i80\_d10 &      224.77 &      276.83 &      262.11 &       311.67 &       366.44 &       402.90 &       403.93 &       373.39 &       384.28 &         405.59 &       319.27 \\ \hline
 f003\_i71\_d05 &      -19.84 &       -1.53 &       -5.36 &         4.79 &        31.46 &        16.91 &         6.41 &        39.46 &        18.86 &          14.00 &        17.47 \\ \hline
 f010\_i75\_d05 &     5675.85 &     3088.20 &    13417.37 &      1697.27 &     11198.30 &      1736.34 &     10378.31 &      5845.49 &      7438.72 &       13534.57 &     60040.98 \\ \hline
 f024\_i79\_d05 &     -960.75 &     -970.10 &     -973.32 &      -966.29 &      -967.61 &      -974.43 &      -956.31 &      -965.85 &      -961.30 &        -958.88 &      -954.23 \\ \hline
 f012\_i03\_d02 &      861.65 &       56.85 &       68.08 &       517.72 &        80.14 &       171.16 &    188411.53 &     69599.82 &   2090941.50 &        6442.20 &       170.61 \\ \hline
 f017\_i76\_d05 &       48.29 &       47.85 &       48.07 &        49.86 &        48.76 &        49.87 &        49.32 &        49.51 &        48.88 &          48.95 &        50.92 \\ \hline
 f024\_i75\_d40 &     -387.96 &     -328.54 &     -531.50 &      -193.43 &      -441.94 &      -426.61 &      -490.57 &      -425.05 &      -436.36 &        -432.18 &       176.60 \\ \hline
 f018\_i73\_d40 &       71.95 &       91.49 &       76.81 &        89.07 &        80.20 &        82.07 &        82.39 &        80.34 &        83.71 &          80.34 &        89.15 \\ \hline
 f022\_i01\_d40 &     -930.38 &     -918.97 &     -932.76 &      -921.42 &      -922.12 &      -920.98 &      -921.92 &      -921.16 &      -921.33 &        -923.11 &      -915.53 \\ \hline
 f004\_i03\_d05 &      148.48 &      143.86 &      152.88 &       188.15 &       207.06 &       164.11 &       204.54 &       188.37 &       190.30 &         208.82 &       183.18 \\ \hline
 f005\_i03\_d40 &      481.22 &       70.59 &      327.37 &       593.20 &       749.75 &       750.84 &       767.66 &       762.82 &       788.46 &         778.11 &       639.03 \\ \hline
 f011\_i77\_d03 &     -278.95 &     -328.09 &     -349.71 &      -329.39 &      -304.38 &      -328.10 &      -337.26 &      -334.09 &       299.89 &        -312.39 &      -306.58 \\ \hline
 f020\_i71\_d20 &     -132.75 &     3998.02 &      360.79 &      1661.73 &      6180.48 &      5173.40 &      2288.76 &      8436.30 &      1758.69 &        1954.57 &     44918.88 \\ \hline
 f001\_i01\_d02 &       79.48 &       79.48 &       79.48 &        79.48 &        79.48 &        79.48 &        79.48 &        79.48 &        79.49 &          79.48 &        80.11 \\ \hline
 f002\_i74\_d10 &     7553.17 &     5226.69 &    63994.36 &    143321.94 &    649623.27 &    195235.73 &    488887.46 &    453538.98 &    105881.26 &      307184.10 &    490820.89 \\ \hline
 f023\_i76\_d05 &     -392.06 &     -392.11 &     -391.32 &      -390.45 &      -391.86 &      -391.99 &      -392.20 &      -390.25 &      -390.46 &        -392.52 &      -391.28 \\ \hline
 f003\_i05\_d40 &      960.53 &     1104.06 &      832.47 &      1572.38 &      1549.18 &      1524.18 &      1533.25 &      1503.34 &      1553.77 &        1378.35 &      2411.23 \\ \hline
 f013\_i76\_d40 &     1852.40 &     3048.02 &     1971.96 &      2868.86 &      2656.56 &      2825.83 &      2732.43 &      2728.70 &      2806.67 &        2749.30 &      3499.78 \\ \hline
 f013\_i75\_d05 &       70.77 &       29.91 &       78.71 &       331.72 &       467.54 &       384.88 &       528.26 &       217.55 &       531.81 &         355.30 &       244.83 \\ \hline
 f017\_i72\_d10 &      -31.23 &      -32.45 &      -30.15 &       -21.66 &       -22.79 &       -25.81 &       -23.28 &       -20.93 &       -22.18 &         -21.26 &       -26.33 \\ \hline
 f013\_i73\_d03 &      -41.01 &      -50.00 &      -38.08 &       -45.55 &       130.36 &       -30.46 &       -38.80 &        50.09 &        -2.97 &           3.67 &        12.19 \\ \hline
 f014\_i03\_d03 &       77.32 &       77.32 &       77.32 &        77.38 &        77.51 &        77.43 &        77.38 &        77.34 &        77.43 &          77.35 &        77.83 \\ \hline
 f004\_i01\_d05 &     -427.52 &     -429.17 &     -421.75 &      -441.52 &      -412.64 &      -409.70 &      -387.09 &      -419.41 &      -404.64 &        -407.95 &      -386.38 \\ \hline
 f005\_i75\_d03 &     -102.36 &     -102.62 &     -102.62 &       -75.39 &       -81.32 &       -85.62 &       -68.44 &       -71.16 &       -87.41 &         -72.07 &       -94.49 \\ \hline
 f021\_i71\_d03 &      -85.26 &      -85.38 &      -84.42 &       -86.28 &       -83.66 &       -84.17 &       -84.75 &       -84.04 &       -84.00 &         -84.16 &       -84.09 \\ \hline
 f018\_i80\_d20 &       61.10 &       63.43 &       60.72 &        67.30 &        62.74 &        71.74 &        68.52 &        70.11 &        74.48 &          66.04 &        83.10 \\ \hline
 f001\_i03\_d02 &     -247.10 &     -247.11 &     -247.11 &      -246.70 &      -246.84 &      -247.04 &      -247.11 &      -247.06 &      -246.90 &        -245.13 &      -247.08 \\ \hline
 f024\_i74\_d02 &       35.22 &       39.18 &       43.04 &        39.76 &        34.68 &        36.52 &        37.49 &        39.03 &        40.00 &          41.02 &        39.70 \\ \hline
 f007\_i72\_d40 &      868.25 &     1225.96 &      748.39 &      1661.32 &      1659.30 &      1388.97 &      1496.48 &      1532.74 &      1755.53 &        1578.22 &      1872.05 \\ \hline
 f012\_i79\_d10 &  1252291.05 &  4646358.57 &  4904448.86 &  23499035.33 &  32367763.09 &  25540736.37 &  22782920.59 &  25679834.93 &  24019008.95 &    26447144.31 &  18294462.44 \\ \hline
 f011\_i78\_d02 &        6.85 &        3.79 &       -2.30 &         0.47 &     59752.78 &       432.71 &      2917.29 &     11640.16 &   1049495.82 &       35169.25 &      3484.59 \\ \hline
 f002\_i73\_d05 &      529.12 &        9.25 &     1282.86 &      1594.69 &    188775.15 &     49741.42 &    153197.17 &     76680.72 &     43849.25 &      132091.57 &     64003.80 \\ \hline
 f017\_i05\_d10 &     -144.83 &     -145.17 &     -144.45 &      -143.50 &      -143.85 &      -143.66 &      -143.32 &      -144.42 &      -143.66 &        -143.89 &      -138.21 \\ \hline
 f009\_i74\_d40 &    13877.53 &      285.47 &    21193.64 &    103524.42 &      3780.06 &      3597.44 &      3926.53 &      3904.40 &      3355.42 &        4086.08 &    211956.15 \\ \hline
 f016\_i73\_d20 &      760.28 &      761.01 &      769.46 &       757.01 &       771.65 &       761.89 &       767.65 &       761.87 &       774.49 &         766.13 &       774.75 \\ \hline
 f018\_i02\_d05 &       20.56 &       20.04 &       21.94 &        23.52 &        21.28 &        28.99 &        26.58 &        24.35 &        27.43 &          24.72 &        36.69 \\ \hline
 f023\_i79\_d40 &      -51.80 &      -52.03 &      -50.86 &       -52.14 &       -53.38 &       -52.57 &       -54.36 &       -52.96 &       -53.12 &         -51.95 &       -51.67 \\ \hline
 f004\_i75\_d05 &      -32.14 &      -20.30 &      -27.64 &       -11.63 &        25.12 &        40.68 &        37.53 &        30.52 &        35.49 &          36.07 &        53.95 \\ \hline
 f023\_i78\_d40 &      144.88 &      145.55 &      146.42 &       145.97 &       145.44 &       143.97 &       144.41 &       145.88 &       144.45 &         145.28 &       145.85 \\ \hline
 f019\_i80\_d20 &       43.71 &       35.59 &       45.56 &        41.15 &        41.66 &        41.88 &        42.16 &        42.70 &        41.92 &          41.31 &        59.61 \\ \hline
 f001\_i75\_d05 &      -25.12 &      -25.31 &      -23.82 &       -18.01 &       -16.91 &       -11.18 &        -8.56 &       -14.16 &        -5.42 &          -9.32 &       -18.08 \\ \hline
 f018\_i04\_d05 &       39.06 &       65.02 &       43.59 &        46.28 &        60.61 &        56.29 &        64.35 &        68.14 &        60.11 &          60.58 &        58.07 \\ \hline
 f003\_i76\_d10 &     -533.04 &     -552.12 &     -508.13 &      -501.25 &      -504.94 &      -462.04 &      -465.85 &      -514.16 &      -518.50 &        -464.41 &      -404.32 \\ \hline
 f015\_i79\_d10 &     -291.72 &     -226.53 &     -282.19 &      -256.61 &      -223.97 &      -245.46 &      -198.31 &      -218.01 &      -223.71 &        -219.15 &      -128.68 \\ \hline
 f018\_i03\_d10 &      284.71 &      307.87 &      293.04 &       305.09 &       319.90 &       320.96 &       319.66 &       311.47 &       320.34 &         322.67 &       308.86 \\ \hline
 f012\_i76\_d03 &     1588.91 &       -0.49 &      268.12 &     82031.37 &    113507.76 &    156584.81 &   1828908.33 &    460662.90 &   3918274.22 &     2833689.73 &     21457.54 \\ \hline
 f016\_i73\_d05 &      735.00 &      734.42 &      739.82 &       738.78 &       753.10 &       744.27 &       749.14 &       749.17 &       743.47 &         747.96 &       747.47 \\ \hline
 f009\_i73\_d02 &     1000.26 &     1000.24 &     1000.30 &      1000.00 &      1000.02 &      1000.07 &      1000.21 &      1000.16 &      1000.08 &        1000.00 &      1004.45 \\ \hline
 f007\_i77\_d05 &      -12.45 &      -11.91 &       -9.34 &        18.44 &        -1.58 &        -1.93 &         2.91 &        19.34 &        10.22 &           5.64 &        -1.54 \\ \hline
 f001\_i80\_d40 &       22.16 &      150.80 &       24.40 &       143.78 &       110.09 &       118.84 &       110.23 &        88.48 &       102.54 &         103.42 &       267.85 \\ \hline
 f021\_i74\_d10 &     -325.09 &     -322.07 &     -314.76 &      -309.85 &      -307.30 &      -293.01 &      -292.62 &      -295.81 &      -304.46 &        -305.01 &      -272.48 \\ \hline
 f005\_i05\_d02 &      -37.36 &      -37.45 &      -37.45 &       -35.31 &       -35.99 &       -35.81 &       -19.91 &       -23.16 &       -14.40 &         -14.85 &       -35.48 \\ \hline
 f014\_i03\_d40 &      102.92 &      133.34 &      100.04 &       127.70 &       113.97 &       114.11 &       112.28 &       110.08 &       111.15 &         109.73 &       178.96 \\ \hline
 f021\_i04\_d40 &       29.90 &       48.71 &       31.50 &        44.31 &        43.96 &        44.72 &        45.06 &        44.95 &        44.47 &          44.65 &        50.99 \\ \hline
 f006\_i79\_d10 &      685.94 &      669.77 &      740.50 &    104063.32 &    210450.37 &    120359.38 &    180246.55 &    109009.07 &    181972.92 &      130230.49 &    134998.92 \\ \hline
 f018\_i79\_d02 &      733.28 &      733.05 &      733.71 &       820.76 &       733.50 &       737.50 &       735.01 &       733.71 &       742.29 &         778.13 &       734.32 \\ \hline
 f015\_i71\_d05 &     -326.30 &     -333.02 &     -335.87 &      -307.90 &      -271.04 &      -299.50 &      -280.51 &      -283.03 &      -318.52 &        -288.63 &      -290.25 \\ \hline
 f007\_i76\_d03 &       49.73 &       49.54 &       52.99 &        49.56 &       138.39 &        58.07 &        50.43 &        51.22 &        75.56 &         108.49 &        63.66 \\ \hline
 f007\_i77\_d10 &       -1.04 &       27.69 &        8.26 &        37.05 &        33.10 &        55.09 &        71.01 &        37.16 &        52.83 &          73.39 &       198.51 \\ \hline
 f019\_i71\_d03 &       62.11 &       61.95 &       63.54 &        62.18 &        62.24 &        62.42 &        62.56 &        62.56 &        62.52 &          63.07 &        63.48 \\ \hline
 f002\_i72\_d05 &     -131.52 &     -334.47 &     4713.44 &     78782.42 &    222589.14 &    246938.52 &    219145.84 &    123738.60 &    264823.07 &      156082.36 &     15500.45 \\ \hline
 f012\_i76\_d05 &   184862.32 &    74983.57 &   433321.32 &    434448.23 &   6866380.89 &   2700650.00 &   6576576.03 &   4591230.30 &   3039001.30 &     9633690.92 &   7160524.92 \\ \hline
 f004\_i71\_d05 &      -16.11 &       10.52 &       -7.89 &         3.98 &         4.92 &        18.35 &        22.04 &         2.51 &        48.04 &           9.34 &        53.63 \\ \hline
 Geometric Mean &        7.50 &       12.50 &       21.30 &        72.30 &        97.80 &       107.00 &       107.40 &       111.50 &       124.30 &         131.10 &       183.80 \\ \hline
\bottomrule
\end{tabular}


==> tables/results_ensemble.tex <==
\begin{tabular}{|lrrrrrrrrrr|}
\toprule
       instance &    HPFSO &         CMA &  best per method &     GBM-LCB &  random-subselection &         GGA++ &       TUR &  RER &  REP &         LHS \\ \hline
\midrule
 f016\_i04\_d05 &    -512.05 &     -503.08 &          -501.34 &     -510.31 &              -507.42 &     -509.37 &     -507.93 &                   -508.65 &                    -505.83 &     -502.32 \\ \hline
 f020\_i80\_d40 &    2633.91 &     8488.18 &         34351.12 &   119145.70 &             39245.08 &   153613.58 &   132934.19 &                 135607.79 &                  101917.84 &   101864.68 \\ \hline
 f008\_i01\_d03 &     151.55 &      151.28 &           154.98 &      350.13 &               198.12 &      277.75 &      347.54 &                    165.61 &                     230.19 &      479.84 \\ \hline
 f017\_i74\_d10 &     -30.35 &      -27.95 &           -25.42 &      -27.41 &               -26.37 &      -21.22 &      -19.53 &                    -19.71 &                     -15.55 &      -16.35 \\ \hline
 f018\_i05\_d05 &    -145.98 &     -143.76 &          -125.09 &     -143.88 &              -139.04 &     -122.54 &     -125.56 &                   -133.14 &                    -128.25 &     -127.76 \\ \hline
 f018\_i04\_d40 &      71.63 &       84.76 &            81.75 &       80.97 &                80.78 &      111.45 &       99.40 &                    103.60 &                     117.21 &      110.97 \\ \hline
 f005\_i77\_d03 &     150.82 &      149.59 &           150.68 &      149.88 &               150.71 &      161.35 &      163.40 &                    160.18 &                     159.02 &      160.94 \\ \hline
 f002\_i72\_d20 &  158102.01 &  1460471.44 &        921442.46 &   401311.91 &            952984.13 &  1760264.92 &  2299094.08 &                3607791.78 &                 4356373.66 &  2217764.86 \\ \hline
 f012\_i01\_d03 &    1151.89 &     -520.09 &         45762.30 &      186.45 &              3099.39 &    90179.63 &   565158.68 &                 454332.24 &                  163686.53 &     6282.28 \\ \hline
 f019\_i04\_d10 &     -54.81 &      -52.82 &           -58.23 &      -48.24 &               -51.23 &      -44.45 &      -47.49 &                    -44.33 &                     -47.21 &      -48.01 \\ \hline
 f020\_i01\_d03 &    -544.73 &     -544.26 &          -544.43 &     -544.83 &              -544.78 &     -543.83 &     -543.04 &                   -542.07 &                    -543.76 &     -544.35 \\ \hline
 f015\_i80\_d20 &     404.78 &      428.70 &           683.35 &      499.16 &               536.39 &      851.25 &      979.57 &                    608.11 &                     847.65 &     1019.94 \\ \hline
 f008\_i76\_d10 &    1194.40 &     1220.85 &          3873.09 &     2307.21 &              4955.09 &    37261.64 &    40566.46 &                  57016.49 &                   14530.10 &    23955.79 \\ \hline
 f020\_i05\_d02 &      -5.74 &       -5.02 &            -5.45 &       -5.11 &                -5.03 &       -3.10 &       -5.35 &                     -4.02 &                      -6.14 &       -3.32 \\ \hline
 f010\_i77\_d05 &    5457.04 &     1720.34 &        285974.44 &     1667.81 &             27924.43 &   472519.76 &    83927.63 &                 149829.04 &                  180905.94 &   282228.52 \\ \hline
 f010\_i74\_d20 &  210079.29 &   726094.08 &        752084.84 &   844504.46 &            805392.77 &  1794493.17 &  1092779.77 &                1241507.12 &                 1740241.83 &  1967016.57 \\ \hline
 f009\_i05\_d40 &    9078.92 &     9257.76 &           319.11 &   218898.52 &             43964.58 &   243943.64 &   300558.93 &                 246345.54 &                  294076.08 &   314224.32 \\ \hline
 f011\_i76\_d40 &     196.24 &     2142.53 &           343.06 &      492.70 &              8165.83 &      427.59 &      376.64 &                    679.54 &                    2391.94 &     3088.82 \\ \hline
 f007\_i05\_d02 &      64.80 &       64.80 &            65.42 &       67.30 &                65.05 &       64.83 &       64.90 &                     66.77 &                      66.40 &       66.77 \\ \hline
 f014\_i04\_d02 &      39.92 &       39.92 &            40.12 &       39.92 &                40.12 &       40.24 &       40.28 &                     39.98 &                      40.24 &       40.45 \\ \hline
 f010\_i05\_d05 &     241.08 &    40305.49 &         83265.80 &     3348.68 &             18943.34 &    33672.07 &    19758.39 &                  46264.82 &                  201996.79 &   155835.22 \\ \hline
 f004\_i76\_d40 &     636.84 &      661.01 &           797.53 &     1651.06 &              1345.54 &     2355.06 &     2172.42 &                   2128.08 &                    3170.98 &     2224.07 \\ \hline
 f018\_i76\_d05 &      50.15 &       54.66 &            56.17 &       56.32 &                64.39 &       71.31 &       55.93 &                     68.63 &                      67.45 &       69.52 \\ \hline
 f022\_i71\_d03 &     154.67 &      152.83 &           155.61 &      158.75 &               153.04 &      155.64 &      159.61 &                    152.81 &                     158.62 &      154.88 \\ \hline
 f014\_i74\_d02 &       7.73 &        7.64 &             7.68 &        7.64 &                 7.70 &        7.82 &        7.87 &                      7.80 &                       8.29 &        8.43 \\ \hline
 f022\_i05\_d10 &      70.41 &       78.66 &           112.29 &      117.98 &               102.73 &      122.27 &      117.82 &                    116.26 &                     114.90 &      121.63 \\ \hline
 f010\_i73\_d10 &   23265.86 &   206082.31 &        153650.36 &   254780.09 &            140428.34 &   281368.69 &   942759.21 &                 263231.20 &                  303966.03 &   563575.33 \\ \hline
 f013\_i71\_d02 &      29.09 &       28.52 &            33.52 &       46.02 &                39.33 &       43.93 &       33.70 &                     78.89 &                      45.82 &       29.65 \\ \hline
 f020\_i73\_d10 &    -245.16 &     -244.70 &          -243.11 &     2286.62 &              2292.53 &     7825.83 &     9341.85 &                   3619.01 &                    6268.29 &     6466.41 \\ \hline
 f008\_i79\_d40 &   38013.69 &    65611.22 &         54010.50 &   110635.08 &            155787.46 &   458041.36 &   283658.51 &                 434738.61 &                  373969.26 &   183046.50 \\ \hline
 f001\_i73\_d40 &    -514.39 &     -479.46 &          -405.13 &     -363.43 &              -401.51 &     -307.30 &     -281.91 &                   -255.49 &                    -272.43 &     -286.93 \\ \hline
 f006\_i01\_d02 &      35.98 &       35.90 &            40.02 &       45.26 &                37.05 &       38.18 &       36.24 &                     36.62 &                      36.35 &       36.58 \\ \hline
 f010\_i79\_d02 &    -986.01 &     -962.71 &          -502.32 &     -982.54 &               184.54 &     -908.74 &     -971.75 &                   -622.81 &                    -620.20 &    11548.17 \\ \hline
 f010\_i76\_d20 &  372372.36 &  1075721.58 &        765021.34 &  2810079.21 &            594062.91 &  2752308.00 &  2573125.36 &                1767184.78 &                 2061908.83 &  1637939.80 \\ \hline
 f004\_i74\_d40 &     808.33 &     1227.10 &          1145.78 &     2307.44 &              1684.73 &     3190.52 &     2858.47 &                   2599.13 &                    2563.06 &     2526.26 \\ \hline
 f008\_i78\_d10 &    1047.95 &     1176.76 &          2200.50 &     5862.26 &              4876.76 &     5594.44 &    17146.04 &                   7176.77 &                   21620.30 &    10275.80 \\ \hline
 f008\_i77\_d03 &    -676.89 &     -678.92 &          -652.42 &     -676.99 &              -671.61 &     -537.22 &     -465.54 &                   -667.45 &                    -675.47 &     -456.59 \\ \hline
 f022\_i80\_d02 &    -305.86 &     -305.86 &          -306.52 &     -305.79 &              -305.69 &     -306.55 &     -306.02 &                   -306.06 &                    -304.45 &     -304.73 \\ \hline
 f005\_i05\_d10 &     -16.97 &      -31.57 &            17.88 &       -5.75 &               -10.13 &       70.54 &       35.68 &                     43.91 &                      69.76 &       78.19 \\ \hline
 f018\_i04\_d10 &      49.66 &       53.05 &            50.00 &       51.69 &                55.77 &       66.55 &       60.89 &                     64.92 &                      69.81 &       60.21 \\ \hline
 f006\_i80\_d10 &     -82.84 &      450.67 &          1844.57 &      -52.33 &                35.64 &    65192.23 &    61142.58 &                  95950.95 &                   34755.77 &    33864.33 \\ \hline
 f008\_i72\_d10 &     -54.56 &      462.32 &          2308.65 &    11742.76 &               682.35 &    14943.61 &     7906.45 &                  26603.86 &                   13042.15 &    13490.75 \\ \hline
 f013\_i77\_d40 &    2122.71 &     2076.70 &          3177.61 &     3424.19 &              2757.78 &     3670.78 &     3257.58 &                   3509.41 &                    3450.73 &     3758.63 \\ \hline
 f007\_i03\_d05 &       6.74 &        7.36 &            12.19 &        9.16 &                 5.32 &       13.44 &       33.35 &                     34.33 &                      29.33 &       28.21 \\ \hline
 f010\_i01\_d03 &     115.04 &      -17.71 &         16389.45 &    16035.43 &               -44.70 &     6122.50 &    10067.99 &                   9959.54 &                    4301.74 &      952.09 \\ \hline
 f013\_i80\_d03 &     -41.36 &       -8.53 &            26.47 &      -36.34 &                 3.75 &      120.66 &       51.55 &                     26.48 &                      89.01 &       49.93 \\ \hline
 f003\_i01\_d03 &    -459.82 &     -454.87 &          -450.00 &     -458.73 &              -455.30 &     -454.76 &     -444.39 &                   -436.59 &                    -436.14 &     -431.29 \\ \hline
 f011\_i78\_d40 &     347.11 &     2668.35 &           408.77 &     3637.31 &              2780.29 &     1063.97 &      964.83 &                    598.57 &                     424.50 &     2166.89 \\ \hline
 f009\_i71\_d02 &     935.02 &      935.57 &           935.08 &      936.02 &               935.06 &      935.80 &      936.31 &                    935.11 &                     935.85 &      940.09 \\ \hline
 f019\_i03\_d40 &     224.37 &      226.03 &           214.26 &      246.72 &               229.73 &      242.24 &      243.35 &                    241.37 &                     243.70 &      246.89 \\ \hline
 f023\_i72\_d20 &    1004.32 &     1007.78 &          1005.05 &     1004.60 &              1003.76 &     1006.50 &     1004.97 &                   1005.63 &                    1004.61 &     1005.09 \\ \hline
 f022\_i01\_d05 &    -999.51 &     -998.00 &          -981.30 &     -983.18 &              -991.47 &     -995.56 &     -973.74 &                   -975.76 &                    -967.34 &     -997.74 \\ \hline
 f005\_i80\_d03 &     -40.47 &      -40.96 &           -38.92 &      -40.59 &               -40.06 &      -28.98 &      -31.71 &                    -33.98 &                     -32.89 &      -32.11 \\ \hline
 f013\_i79\_d40 &    1256.77 &     1470.50 &          2004.30 &     2347.72 &              2123.35 &     2792.58 &     3037.91 &                   2974.26 &                    3020.75 &     2907.08 \\ \hline
 f010\_i02\_d10 &   96356.82 &    16730.76 &        233558.50 &   132218.76 &            113231.80 &   398890.88 &   356654.12 &                 286796.16 &                  264542.67 &   739880.47 \\ \hline
 f023\_i03\_d10 &    -127.20 &     -126.06 &          -127.93 &     -127.38 &              -128.37 &     -127.42 &     -126.50 &                   -128.08 &                    -127.39 &     -126.68 \\ \hline
 f022\_i03\_d10 &     -45.44 &      -22.10 &            17.59 &       -9.74 &                11.28 &       21.90 &       11.25 &                     13.89 &                      16.91 &      -30.34 \\ \hline
 f007\_i80\_d10 &    1012.62 &     1047.83 &          1056.68 &     1118.55 &              1055.23 &     1137.41 &     1048.93 &                   1100.49 &                    1160.38 &     1105.26 \\ \hline
 f016\_i01\_d10 &      91.06 &       96.60 &           101.86 &       98.37 &                91.95 &       83.81 &      106.00 &                     99.29 &                      90.84 &       93.29 \\ \hline
 f005\_i74\_d02 &    -182.61 &     -183.02 &          -182.79 &     -182.97 &              -182.84 &     -176.11 &     -180.85 &                   -180.81 &                    -180.40 &     -176.14 \\ \hline
 f007\_i05\_d40 &     443.28 &      828.50 &          1384.91 &     1316.82 &              1216.25 &     1920.17 &     2092.79 &                   2447.89 &                    1719.92 &     2041.27 \\ \hline
 f006\_i04\_d02 &     133.06 &      132.25 &           135.13 &      143.82 &               140.11 &      132.73 &      133.21 &                    134.04 &                     135.18 &      140.78 \\ \hline
 f022\_i74\_d20 &      51.11 &       81.36 &            91.18 &       89.52 &                89.14 &       93.75 &       92.15 &                     92.45 &                      92.83 &       93.98 \\ \hline
 f011\_i79\_d40 &     724.00 &      541.81 &           592.71 &      927.31 &              3611.33 &      727.75 &    28333.59 &                   4846.74 &                    2443.46 &      811.81 \\ \hline
 f013\_i02\_d05 &      12.46 &       10.98 &           251.84 &       48.15 &                93.66 &      353.08 &      427.71 &                    356.13 &                      94.99 &      357.82 \\ \hline
 f010\_i05\_d10 &   35412.80 &   110867.95 &        231107.18 &    91472.22 &            357975.75 &   315997.77 &   370887.79 &                 879843.85 &                  461416.15 &   225743.02 \\ \hline
 f015\_i78\_d03 &      63.89 &       59.94 &            60.78 &       52.54 &                66.72 &       70.44 &       81.49 &                     74.46 &                      81.54 &       77.17 \\ \hline
 f002\_i05\_d20 &  137401.76 &   676400.15 &       1041336.56 &   296505.24 &            995133.58 &  3097120.29 &  1469275.83 &                1556871.88 &                 2392201.00 &  3791442.16 \\ \hline
 f021\_i01\_d05 &      42.21 &       42.83 &            47.12 &       43.58 &                42.78 &       50.04 &       57.15 &                     44.45 &                      48.98 &       58.26 \\ \hline
 f015\_i79\_d02 &    -362.47 &     -362.23 &          -361.28 &     -355.12 &              -357.11 &     -359.34 &     -359.43 &                   -354.83 &                    -359.73 &     -348.35 \\ \hline
 f013\_i74\_d40 &    1612.80 &     1363.01 &          2560.49 &     2622.84 &              2258.53 &     3213.70 &     3381.94 &                   3521.67 &                    3186.97 &     3092.68 \\ \hline
 f013\_i75\_d10 &     176.58 &      336.53 &           584.30 &      832.89 &               561.73 &      669.98 &      755.66 &                   1083.83 &                     953.39 &     1107.80 \\ \hline
 f009\_i76\_d20 &    1254.15 &     1581.05 &           118.66 &    52298.27 &             18405.01 &    52670.09 &    78978.76 &                 103405.05 &                   93726.41 &    95257.94 \\ \hline
 f014\_i02\_d03 &    -179.50 &     -179.40 &          -178.90 &     -178.66 &              -179.37 &     -179.42 &     -178.76 &                   -179.45 &                    -178.52 &     -178.40 \\ \hline
 f005\_i04\_d10 &     956.55 &      941.67 &          1001.16 &      973.42 &               980.01 &     1023.87 &     1052.34 &                   1054.42 &                    1053.14 &     1052.50 \\ \hline
 f013\_i80\_d20 &     702.12 &      833.15 &          1666.48 &     1281.90 &              1299.77 &     1768.91 &     2006.95 &                   1958.15 &                    1944.42 &     2001.39 \\ \hline
 f010\_i03\_d10 &   11948.15 &    56529.06 &        190656.34 &   258770.02 &            120082.81 &   244268.89 &   393889.54 &                 242175.26 &                  548323.89 &   303533.91 \\ \hline
 f009\_i71\_d10 &     976.63 &     1219.03 &           993.32 &     4469.85 &              4913.70 &     6871.93 &    13984.32 &                  13479.02 &                   13570.91 &    19729.36 \\ \hline
 f019\_i79\_d02 &      29.12 &       28.85 &            28.84 &       29.25 &                29.05 &       28.96 &       28.98 &                     28.82 &                      29.02 &       30.53 \\ \hline
\bottomrule
\end{tabular}


==> tables/results_ensemble_cont.tex <==
\begin{tabular}{|l|rrrrrrrrrr|}
\toprule
\hline
       instance &    HPFSO &         CMA &  best per method &     GBM-LCB &  random-subselection &         GGA++ &       TUR &  RER &  REP &         LHS \\ \hline
\midrule
\hline
 f024\_i77\_d02 &       -9.03 &       -9.82 &            -8.42 &       -2.33 &                -6.91 &        -6.98 &        -5.45 &                     -8.74 &                      -5.92 &        -8.12 \\ \hline
 f014\_i74\_d40 &       38.93 &       38.55 &            44.84 &       52.17 &                58.44 &        95.72 &        79.60 &                     78.30 &                     102.66 &       101.39 \\ \hline
 f015\_i02\_d40 &      923.10 &     1002.62 &          1373.10 &     1485.66 &              1360.65 &      2006.42 &      2208.74 &                   2359.70 &                    1497.33 &      1938.79 \\ \hline
 f005\_i02\_d03 &      656.22 &      655.99 &           656.51 &      656.62 &               656.69 &       663.38 &       662.76 &                    673.52 &                     665.25 &       666.09 \\ \hline
 f019\_i77\_d20 &       -3.96 &       -1.55 &           -10.10 &        4.83 &                 1.87 &         7.14 &        14.12 &                      4.61 &                      13.26 &         7.32 \\ \hline
 f002\_i04\_d02 &      320.31 &      320.24 &           373.33 &      327.08 &               478.92 &      1534.65 &       413.13 &                  29266.26 &                    9538.62 &    230437.67 \\ \hline
 f012\_i72\_d02 &      -39.33 &      -85.21 &            71.25 &      -41.64 &               -39.33 &      4541.76 &       -84.90 &                    390.27 &                    1726.89 &       120.91 \\ \hline
 f007\_i74\_d05 &       93.49 &       94.18 &           101.62 &      102.58 &               108.32 &       100.76 &       105.34 &                    152.13 &                     104.89 &       124.12 \\ \hline
 f011\_i01\_d20 &      279.50 &      391.25 &           855.04 &      666.37 &               456.14 &       394.41 &       332.20 &                   1773.97 &                    1274.37 &       645.30 \\ \hline
 f014\_i74\_d10 &        9.86 &       12.80 &            14.30 &       18.32 &                14.26 &        23.04 &        27.90 &                     17.54 &                      24.98 &        18.36 \\ \hline
 f004\_i80\_d20 &      366.28 &      519.06 &           728.85 &      579.14 &               687.11 &       819.53 &      1092.20 &                   1130.14 &                     867.73 &       950.85 \\ \hline
 f014\_i71\_d40 &       65.53 &       54.74 &            98.76 &      132.61 &                94.95 &       133.28 &        98.94 &                    121.27 &                     117.58 &       134.23 \\ \hline
 f019\_i77\_d40 &       -0.48 &        0.89 &           -10.10 &       23.70 &                 2.62 &        19.33 &        16.03 &                     17.65 &                      15.40 &        18.95 \\ \hline
 f017\_i72\_d05 &      -34.58 &      -35.74 &           -30.17 &      -33.37 &               -34.01 &       -32.14 &       -30.98 &                    -32.11 &                     -29.06 &       -30.78 \\ \hline
 f015\_i80\_d10 &      224.77 &      262.11 &           283.22 &      291.22 &               253.99 &       368.03 &       319.27 &                    437.88 &                     364.02 &       433.69 \\ \hline
 f003\_i71\_d05 &      -19.84 &       -5.36 &            15.30 &      -15.99 &                -7.16 &        30.32 &        17.47 &                     13.66 &                      12.39 &        35.47 \\ \hline
 f010\_i75\_d05 &     5675.85 &    13417.37 &          6438.57 &    10906.69 &             18344.35 &     45690.65 &     60040.98 &                  65059.52 &                   26357.25 &     24149.57 \\ \hline
 f024\_i79\_d05 &     -960.75 &     -973.32 &          -973.40 &     -970.59 &              -961.73 &      -942.42 &      -954.23 &                   -945.71 &                    -953.22 &      -944.23 \\ \hline
 f012\_i03\_d02 &      861.65 &       68.08 &          2386.87 &       66.56 &               862.75 &       155.58 &       170.61 &                    958.96 &                     638.36 &      3099.27 \\ \hline
 f017\_i76\_d05 &       48.29 &       48.07 &            49.54 &       51.03 &                51.57 &        53.54 &        50.92 &                     53.60 &                      50.71 &        52.79 \\ \hline
 f024\_i75\_d40 &     -387.96 &     -531.50 &          -442.83 &       82.63 &              -210.12 &       323.09 &       176.60 &                    249.85 &                     366.84 &       137.74 \\ \hline
 f018\_i73\_d40 &       71.95 &       76.81 &            86.61 &      101.73 &                97.75 &       100.08 &        89.15 &                     96.17 &                     113.37 &        97.06 \\ \hline
 f022\_i01\_d40 &     -930.38 &     -932.76 &          -920.60 &     -915.50 &              -920.49 &      -915.06 &      -915.53 &                   -917.39 &                    -917.48 &      -915.11 \\ \hline
 f004\_i03\_d05 &      148.48 &      152.88 &           201.96 &      138.43 &               171.30 &       194.33 &       183.18 &                    180.98 &                     198.85 &       220.18 \\ \hline
 f005\_i03\_d40 &      481.22 &      327.37 &           596.14 &      479.62 &               454.36 &       631.10 &       639.03 &                    669.57 &                     642.37 &       664.64 \\ \hline
 f011\_i77\_d03 &     -278.95 &     -349.71 &          -318.53 &     -313.15 &               949.41 &      2405.84 &      -306.58 &                   -307.26 &                     899.36 &     10823.72 \\ \hline
 f020\_i71\_d20 &     -132.75 &      360.79 &          4837.51 &    22995.70 &             10866.23 &     29506.09 &     44918.88 &                  31740.46 &                   15418.35 &     59569.89 \\ \hline
 f001\_i01\_d02 &       79.48 &       79.48 &            79.48 &       79.49 &                79.49 &        80.49 &        80.11 &                     79.54 &                      79.69 &        80.13 \\ \hline
 f002\_i74\_d10 &     7553.17 &    63994.36 &        145154.25 &    16605.68 &            117592.55 &    286504.75 &    490820.89 &                 451817.00 &                  598420.65 &    495388.93 \\ \hline
 f023\_i76\_d05 &     -392.06 &     -391.32 &          -390.67 &     -390.40 &              -392.72 &      -390.26 &      -391.28 &                   -389.37 &                    -391.44 &      -391.76 \\ \hline
 f003\_i05\_d40 &      960.53 &      832.47 &          1554.23 &     1394.52 &              1201.16 &      2065.06 &      2411.23 &                   2598.51 &                    1954.49 &      2130.15 \\ \hline
 f013\_i76\_d40 &     1852.40 &     1971.96 &          2885.40 &     3054.85 &              2759.73 &      3029.25 &      3499.78 &                   3704.12 &                    3465.37 &      3589.84 \\ \hline
 f013\_i75\_d05 &       70.77 &       78.71 &           242.78 &      102.76 &               136.16 &       500.86 &       244.83 &                    402.31 &                     323.15 &       348.72 \\ \hline
 f017\_i72\_d10 &      -31.23 &      -30.15 &           -28.61 &      -31.31 &               -30.53 &       -25.46 &       -26.33 &                    -22.50 &                     -21.37 &       -25.98 \\ \hline
 f013\_i73\_d03 &      -41.01 &      -38.08 &           -33.80 &      -38.23 &               -13.49 &        44.11 &        12.19 &                     77.38 &                     120.80 &        49.64 \\ \hline
 f014\_i03\_d03 &       77.32 &       77.32 &            78.03 &       77.32 &                77.75 &        77.72 &        77.83 &                     78.48 &                      77.90 &        78.06 \\ \hline
 f004\_i01\_d05 &     -427.52 &     -421.75 &          -419.13 &     -358.36 &              -375.42 &      -411.75 &      -386.38 &                   -373.47 &                    -374.66 &      -384.74 \\ \hline
 f005\_i75\_d03 &     -102.36 &     -102.62 &          -101.56 &     -102.46 &              -101.81 &       -94.59 &       -94.49 &                    -82.30 &                     -91.39 &       -92.52 \\ \hline
 f021\_i71\_d03 &      -85.26 &      -84.42 &           -84.25 &      -83.75 &               -84.23 &       -84.32 &       -84.09 &                    -82.93 &                     -84.32 &       -81.86 \\ \hline
 f018\_i80\_d20 &       61.10 &       60.72 &            74.74 &       64.91 &                76.39 &        73.70 &        83.10 &                     88.28 &                      86.83 &        89.19 \\ \hline
 f001\_i03\_d02 &     -247.10 &     -247.11 &          -247.10 &     -247.11 &              -247.11 &      -246.84 &      -247.08 &                   -247.10 &                    -246.92 &      -246.60 \\ \hline
 f024\_i74\_d02 &       35.22 &       43.04 &            38.81 &       35.86 &                37.67 &        40.64 &        39.70 &                     38.06 &                      39.06 &        39.86 \\ \hline
 f007\_i72\_d40 &      868.25 &      748.39 &          1576.47 &     1683.97 &              1274.83 &      2534.65 &      1872.05 &                   2705.79 &                    2484.40 &      2639.05 \\ \hline
 f012\_i79\_d10 &  1252291.05 &  4904448.86 &      18121933.07 &  8398428.74 &          31910978.74 &  42737993.63 &  18294462.44 &               50000342.63 &                32935623.05 &  40912799.54 \\ \hline
 f011\_i78\_d02 &        6.85 &       -2.30 &            41.32 &        2.60 &               902.48 &        31.94 &      3484.59 &                   2388.57 &                    2736.18 &     33801.28 \\ \hline
 f002\_i73\_d05 &      529.12 &     1282.86 &         57130.63 &      325.41 &             29865.07 &    100905.49 &     64003.80 &                  12668.79 &                   39037.06 &     29427.18 \\ \hline
 f017\_i05\_d10 &     -144.83 &     -144.45 &          -143.69 &     -142.32 &              -139.46 &      -140.99 &      -138.21 &                   -141.83 &                    -139.74 &      -140.91 \\ \hline
 f009\_i74\_d40 &    13877.53 &    21193.64 &           285.47 &   346005.26 &             71747.12 &    329239.28 &    211956.15 &                 264757.88 &                  273503.67 &    275278.92 \\ \hline
 f016\_i73\_d20 &      760.28 &      769.46 &           768.05 &      768.52 &               771.86 &       765.24 &       774.75 &                    765.74 &                     770.79 &       754.98 \\ \hline
 f018\_i02\_d05 &       20.56 &       21.94 &            26.40 &       26.41 &                27.63 &        31.09 &        36.69 &                     28.89 &                      32.22 &        33.05 \\ \hline
 f023\_i79\_d40 &      -51.80 &      -50.86 &           -52.90 &      -51.06 &               -52.31 &       -51.59 &       -51.67 &                    -53.10 &                     -49.87 &       -50.59 \\ \hline
 f004\_i75\_d05 &      -32.14 &      -27.64 &           -21.07 &      -27.28 &               -31.14 &        29.05 &        53.95 &                     34.62 &                      25.54 &        21.13 \\ \hline
 f023\_i78\_d40 &      144.88 &      146.42 &           146.57 &      146.47 &               147.03 &       147.22 &       145.85 &                    146.90 &                     147.64 &       147.31 \\ \hline
 f019\_i80\_d20 &       43.71 &       45.56 &            35.59 &       52.18 &                46.90 &        53.01 &        59.61 &                     56.18 &                      52.46 &        56.57 \\ \hline
 f001\_i75\_d05 &      -25.12 &      -23.82 &           -23.55 &      -24.82 &               -24.99 &       -15.04 &       -18.08 &                    -17.62 &                     -18.05 &       -23.02 \\ \hline
 f018\_i04\_d05 &       39.06 &       43.59 &            55.07 &       60.25 &                45.48 &        52.10 &        58.07 &                     54.90 &                      58.06 &        49.42 \\ \hline
 f003\_i76\_d10 &     -533.04 &     -508.13 &          -495.60 &     -479.74 &              -459.77 &      -419.05 &      -404.32 &                   -339.10 &                    -403.32 &      -410.73 \\ \hline
 f015\_i79\_d10 &     -291.72 &     -282.19 &          -240.77 &     -233.52 &              -254.65 &      -110.88 &      -128.68 &                   -170.05 &                     -83.87 &      -134.10 \\ \hline
 f018\_i03\_d10 &      284.71 &      293.04 &           306.43 &      289.67 &               291.58 &       315.10 &       308.86 &                    320.09 &                     317.47 &       321.52 \\ \hline
 f012\_i76\_d03 &     1588.91 &      268.12 &        144148.44 &     1040.16 &            168915.11 &     45100.75 &     21457.54 &                 127315.61 &                   63619.57 &    911058.88 \\ \hline
 f016\_i73\_d05 &      735.00 &      739.82 &           746.39 &      738.81 &               733.06 &       737.97 &       747.47 &                    735.20 &                     745.66 &       740.67 \\ \hline
 f009\_i73\_d02 &     1000.26 &     1000.30 &          1000.80 &     1001.92 &              1001.33 &      1006.94 &      1004.45 &                   1005.53 &                    1000.53 &      1014.34 \\ \hline
 f007\_i77\_d05 &      -12.45 &       -9.34 &            -9.23 &       26.58 &                -5.98 &         7.71 &        -1.54 &                     -0.59 &                      -0.04 &        14.23 \\ \hline
 f001\_i80\_d40 &       22.16 &       24.40 &           111.48 &      204.87 &               101.21 &       269.88 &       267.85 &                    254.96 &                     250.28 &       255.26 \\ \hline
 f021\_i74\_d10 &     -325.09 &     -314.76 &          -297.52 &     -311.19 &              -294.81 &      -272.79 &      -272.48 &                   -281.87 &                    -302.86 &      -269.22 \\ \hline
 f005\_i05\_d02 &      -37.36 &      -37.45 &           -37.39 &      -37.42 &               -37.41 &       -36.33 &       -35.48 &                    -34.71 &                     -32.37 &       -30.58 \\ \hline
 f014\_i03\_d40 &      102.92 &      100.04 &           125.31 &      152.11 &               122.72 &       150.50 &       178.96 &                    171.45 &                     142.29 &       134.03 \\ \hline
 f021\_i04\_d40 &       29.90 &       31.50 &            47.05 &       48.38 &                42.83 &        48.52 &        50.99 &                     51.22 &                      50.83 &        51.38 \\ \hline
 f006\_i79\_d10 &      685.94 &      740.50 &           795.74 &      685.57 &               939.51 &      2069.62 &    134998.92 &                  19993.51 &                    8089.12 &     44598.56 \\ \hline
 f018\_i79\_d02 &      733.28 &      733.71 &           740.36 &      733.55 &               733.46 &       743.72 &       734.32 &                    739.75 &                     735.88 &       734.86 \\ \hline
 f015\_i71\_d05 &     -326.30 &     -335.87 &          -309.55 &     -289.05 &              -310.07 &      -292.21 &      -290.25 &                   -274.99 &                    -266.30 &      -289.05 \\ \hline
 f007\_i76\_d03 &       49.73 &       52.99 &            51.44 &       51.39 &                56.03 &        51.61 &        63.66 &                     53.04 &                      61.06 &        50.09 \\ \hline
 f007\_i77\_d10 &       -1.04 &        8.26 &            58.76 &       30.99 &                22.53 &        87.41 &       198.51 &                     70.90 &                      64.16 &       136.03 \\ \hline
 f019\_i71\_d03 &       62.11 &       63.54 &            62.14 &       62.93 &                63.96 &        63.98 &        63.48 &                     64.31 &                      63.41 &        64.99 \\ \hline
 f002\_i72\_d05 &     -131.52 &     4713.44 &           808.77 &      387.12 &             20126.04 &     21929.42 &     15500.45 &                  11068.15 &                   32121.19 &     91938.13 \\ \hline
 f012\_i76\_d05 &   184862.32 &   433321.32 &       1863652.52 &   136870.68 &           4094966.16 &   5116355.94 &   7160524.92 &                4177435.39 &                 2642490.42 &   7524032.69 \\ \hline
 f004\_i71\_d05 &      -16.11 &       -7.89 &             1.82 &        1.17 &                 5.12 &        55.00 &        53.63 &                     82.63 &                      53.03 &        74.34 \\ \hline
 Geometric Mean &        7.50 &       21.30 &            62.80 &       67.10 &                85.40 &       179.60 &       183.80 &                    200.50 &                     203.70 &       232.40 \\ \hline
\bottomrule
\end{tabular}


==> tables/results_variations.tex <==
\begin{tabular}{|llllll|}
\toprule
              method & (64,8) & (128,16) & (64,4) & (256,16) & (128,4) \\ \hline
\midrule
               HPFSO &   21.6 &      NaN &   13.7 &      NaN &     NaN \\ \hline
                HEBO &   22.7 &     13.1 &   26.2 &      NaN &     NaN \\ \hline
                 CMA &   44.8 &     11.2 &     31 &        3 &    35.4 \\ \hline
                 BPM &     73 &      NaN &   82.9 &      NaN &     NaN \\ \hline
             GBM-LCB &   71.1 &       67 &   94.5 &     37.5 &    19.2 \\ \hline
               shade &  110.3 &     91.5 &  109.7 &     61.3 &    59.1 \\ \hline
          lshadecne* &  103.9 &    110.8 &  112.2 &     67.5 &    71.8 \\ \hline
                 jso &  115.8 &     80.4 &  117.7 &     48.6 &    62.7 \\ \hline
                sade &  123.8 &     81.8 &    124 &     66.2 &      57 \\ \hline
                  de &  134.3 &    100.8 &  132.6 &     75.9 &      67 \\ \hline
              lshade &  136.8 &     81.8 &    139 &     55.9 &      54 \\ \hline
 random-subselection &    108 &      NaN &  140.5 &      NaN &     NaN \\ \hline
             ilshade &  145.5 &     57.4 &  149.7 &     26.9 &    33.5 \\ \hline
               GGA++ &  244.5 &    182.5 &  222.8 &    136.4 &   160.4 \\ \hline
                 REP &  213.2 &    185.4 &  225.2 &    132.7 &   171.3 \\ \hline
                 RER &  244.7 &    157.3 &  234.1 &    152.8 &   165.5 \\ \hline
                 TUR &  236.1 &    176.1 &    244 &    147.4 &   148.4 \\ \hline
                 LHS &  254.5 &    195.2 &  305.2 &    149.5 &   217.5 \\ \hline
\bottomrule
\end{tabular}


==> tables/training_test.tex <==
\begin{tabular}{|lllllllll|}
\toprule
          training &           training &         validation &         validation &         validation &         validation &         validation &         validation &         validation \\ \hline
\midrule
 f001\_i77\_d02 &  f016\_i79\_d10 &  f016\_i04\_d05 &  f018\_i76\_d05 &  f010\_i01\_d03 &  f015\_i78\_d03 &  f011\_i01\_d20 &  f013\_i76\_d40 &  f001\_i75\_d05 \\ \hline
 f003\_i79\_d02 &  f020\_i04\_d10 &  f020\_i80\_d40 &  f022\_i71\_d03 &  f013\_i80\_d03 &  f002\_i05\_d20 &  f014\_i74\_d10 &  f013\_i75\_d05 &  f018\_i04\_d05 \\ \hline
 f005\_i72\_d02 &  f021\_i02\_d10 &  f008\_i01\_d03 &  f014\_i74\_d02 &  f003\_i01\_d03 &  f021\_i01\_d05 &  f004\_i80\_d20 &  f017\_i72\_d10 &  f003\_i76\_d10 \\ \hline
 f011\_i72\_d02 &  f022\_i76\_d10 &  f017\_i74\_d10 &  f022\_i05\_d10 &  f011\_i78\_d40 &  f015\_i79\_d02 &  f014\_i71\_d40 &  f013\_i73\_d03 &  f015\_i79\_d10 \\ \hline
 f018\_i71\_d02 &  f004\_i04\_d20 &  f018\_i05\_d05 &  f010\_i73\_d10 &  f009\_i71\_d02 &  f013\_i74\_d40 &  f019\_i77\_d40 &  f014\_i03\_d03 &  f018\_i03\_d10 \\ \hline
 f001\_i77\_d03 &  f011\_i02\_d20 &  f018\_i04\_d40 &  f013\_i71\_d02 &  f019\_i03\_d40 &  f013\_i75\_d10 &  f017\_i72\_d05 &  f004\_i01\_d05 &  f012\_i76\_d03 \\ \hline
 f002\_i76\_d03 &  f011\_i78\_d20 &  f005\_i77\_d03 &  f020\_i73\_d10 &  f023\_i72\_d20 &  f009\_i76\_d20 &  f015\_i80\_d10 &  f005\_i75\_d03 &  f016\_i73\_d05 \\ \hline
 f005\_i74\_d03 &  f012\_i03\_d20 &  f002\_i72\_d20 &  f008\_i79\_d40 &  f022\_i01\_d05 &  f014\_i02\_d03 &  f003\_i71\_d05 &  f021\_i71\_d03 &  f009\_i73\_d02 \\ \hline
 f010\_i75\_d03 &  f012\_i78\_d20 &  f012\_i01\_d03 &  f001\_i73\_d40 &  f005\_i80\_d03 &  f005\_i04\_d10 &  f010\_i75\_d05 &  f018\_i80\_d20 &  f007\_i77\_d05 \\ \hline
 f012\_i01\_d03 &  f017\_i73\_d20 &  f019\_i04\_d10 &  f006\_i01\_d02 &  f013\_i79\_d40 &  f013\_i80\_d20 &  f024\_i79\_d05 &  f001\_i03\_d02 &  f001\_i80\_d40 \\ \hline
 f012\_i03\_d03 &  f017\_i74\_d20 &  f020\_i01\_d03 &  f010\_i79\_d02 &  f010\_i02\_d10 &  f010\_i03\_d10 &  f012\_i03\_d02 &  f024\_i74\_d02 &  f021\_i74\_d10 \\ \hline
 f013\_i72\_d03 &  f019\_i03\_d20 &  f015\_i80\_d20 &  f010\_i76\_d20 &  f023\_i03\_d10 &  f009\_i71\_d10 &  f017\_i76\_d05 &  f007\_i72\_d40 &  f005\_i05\_d02 \\ \hline
 f014\_i73\_d03 &  f024\_i74\_d20 &  f008\_i76\_d10 &  f004\_i74\_d40 &  f022\_i03\_d10 &  f019\_i79\_d02 &  f024\_i75\_d40 &  f012\_i79\_d10 &  f014\_i03\_d40 \\ \hline
 f001\_i74\_d05 &  f002\_i04\_d40 &  f020\_i05\_d02 &  f008\_i78\_d10 &  f007\_i80\_d10 &  f013\_i79\_d20 &  f018\_i73\_d40 &  f011\_i78\_d02 &  f021\_i04\_d40 \\ \hline
 f002\_i72\_d05 &  f010\_i05\_d40 &  f010\_i77\_d05 &  f008\_i77\_d03 &  f016\_i01\_d10 &  f024\_i77\_d02 &  f022\_i01\_d40 &  f002\_i73\_d05 &  f006\_i79\_d10 \\ \hline
 f004\_i72\_d05 &  f013\_i79\_d40 &  f010\_i74\_d20 &  f022\_i80\_d02 &  f005\_i74\_d02 &  f014\_i74\_d40 &  f004\_i03\_d05 &  f017\_i05\_d10 &  f018\_i79\_d02 \\ \hline
 f008\_i79\_d05 &  f017\_i72\_d40 &  f009\_i05\_d40 &  f005\_i05\_d10 &  f007\_i05\_d40 &  f015\_i02\_d40 &  f005\_i03\_d40 &  f009\_i74\_d40 &  f015\_i71\_d05 \\ \hline
 f013\_i71\_d05 &  f020\_i80\_d40 &  f011\_i76\_d40 &  f018\_i04\_d10 &  f006\_i04\_d02 &  f005\_i02\_d03 &  f011\_i77\_d03 &  f016\_i73\_d20 &  f007\_i76\_d03 \\ \hline
 f016\_i77\_d05 &  f023\_i76\_d40 &  f007\_i05\_d02 &  f006\_i80\_d10 &  f022\_i74\_d20 &  f019\_i77\_d20 &  f020\_i71\_d20 &  f018\_i02\_d05 &  f007\_i77\_d10 \\ \hline
 f019\_i72\_d05 &  f024\_i74\_d40 &  f014\_i04\_d02 &  f008\_i72\_d10 &  f011\_i79\_d40 &  f002\_i04\_d02 &  f001\_i01\_d02 &  f023\_i79\_d40 &  f019\_i71\_d03 \\ \hline
 f023\_i75\_d05 &  f024\_i80\_d40 &  f010\_i05\_d05 &  f013\_i77\_d40 &  f013\_i02\_d05 &  f012\_i72\_d02 &  f002\_i74\_d10 &  f004\_i75\_d05 &  f002\_i72\_d05 \\ \hline
 f010\_i79\_d10 &                    &  f004\_i76\_d40 &  f007\_i03\_d05 &  f010\_i05\_d10 &  f007\_i74\_d05 &  f023\_i76\_d05 &  f023\_i78\_d40 &  f012\_i76\_d05 \\ \hline
                   &                    &                    &                    &                    &                    &  f003\_i05\_d40 &  f019\_i80\_d20 &  f004\_i71\_d05 \\ \hline
\bottomrule
\end{tabular}

